Finding Control Synthesis for Kinematic Shortest Paths

This work presents the analysis of the properties of the shortest path control synthesis for the rigid body system. The systems we focus on in this work have only kinematic constraints. However, even for seemingly simple systems and constraints, the shortest paths for generic rigid body systems were only found recently, especially for 3D systems. Based on the Pontraygon's Maximum Principle (MPM) and Lagrange equations, we present the necessary conditions for optimal switches, which form the control synthesis boundaries. We formally show that the shortest path for nearby configurations will have similar adjoint functions and parameters, i.e., Lagrange multipliers. We further show that the gradients of the necessary condition equation can be used to verify whether a configuration is inside a control synthesis region or on the boundary. We present a procedure to find the shortest kinematic paths and control synthesis, using the gradients of the control constraints. Given the shortest path and the corresponding control sequences, the optimal control sequence for nearby configurations can be derived if and only if they belong to the same control synthesis region. The proposed procedure can work for both 2D and 3D rigid body systems. We use a 2D Dubins vehicle system to verify the correctness of the proposed approach. More verifications and experiments will be presented in the extensions of this work.

==> figs/backup.tex <==
% \begin{definition}
% Define a control synthesis region $\mathcal{P}$ as the connected region where all configurations within this region share the same optimal control sequence to the goal, i.e., following the same control sequence will generate the shortest path to the goal. 
% \end{definition}

% If a configuration is on the switching curve, then there must exist two controls satisfying the necessary conditions for optimality at the same time. What is more, the two controls satisfying the necessary condition must be the same for all configurations on the same switching curve. 

% In the case of a switch between two rotations, let us denote the control $i$ with rotation axis $\hat\omega_i$ through rotation center $r_i$ (and $r_i^R$ in the robot frame), and control $j$ with rotation axis $\hat\omega_j$ through rotation center $r_j$ (and $r_j^R$ in the robot frame). We then have, 
% \begin{eqnarray}
% \vec k\cdot(\hat{\omega}_i\times\vec{r_ig}) + \hat{\omega}_i\cdot\vec{c} = H\\
% \vec k\cdot(\hat{\omega}_j\times\vec{r_jg}) + \hat{\omega}_j\cdot\vec{c} = H 
% \end{eqnarray}

% In the case of a switch between a rotation control $i$ and a translation with velocity director $\vec{v}_j$, we have,  
% \begin{eqnarray}
% \vec k\cdot(\hat{\omega}_i\times\vec{r_ig}) + \hat{\omega}_i\cdot\vec{c} = H \\
% \vec k\cdot \vec{v}_j = H
% \end{eqnarray}
% so that we can have the exact orientations at such switches. At such moments, the $\hat\omega_i$ and $\vec{v}_j$ form the same angle as in the robot frame. 



% omit the $\vec{c}$ in a later section. 
